Constraining Higgs sectors of BSM models -- the case of 95 GeV "Higgs"

In view of lack of the direct experimental evidence for a Beyond the Standard Model (BSM) physics, accommodating a SM-like Higgs boson is on the most important constraints that a BSM model must fulfill. Already for some time the FlexibleSUSY spectrum generator generator allowed for a reliable prediction of masses and decay patterns of the BSM Higgs boson in a large class of user defined supersymmetric and non-supersymmetric models. However, no easy way to compare those predictions with experimental data existed. To that end we present here an interface between FlexibleSUSY and HiggsTools, a computer program assessing in a statistically meaningful way consistency of a BSM Higgs sector with experiments. Motivated by the recent ATLAS and CMS observation of the di-photon excess at a mass of $\sim$95 GeV we demonstrate the capabilities of our framework by investigating whether the observed low mass excesses around 95 GeV seen in the data can be explained as the lightest scalar of the Minimal R-symmetric Supersymmetric Standard Model, without spoiling the SM-like properties of the second-to-lightest state. We also briefly comment on the light dark matter candidate which is a necessarily ingredient of such a setup.

==> tex/bibliography.tex <==
\bibitem{Aad:2012tfa}
  G.~Aad {\it et al.} [ATLAS Collaboration],
  %``Observation of a new particle in the search for the Standard Model Higgs boson with the ATLAS detector at the LHC,''
  Phys.\ Lett.\ B {\bf 716} (2012) 1
  doi:10.1016/j.physletb.2012.08.020
  [arXiv:1207.7214 [hep-ex]].

\bibitem{Chatrchyan:2012xdj}
  S.~Chatrchyan {\it et al.} [CMS Collaboration],
  %``Observation of a new boson at a mass of 125 GeV with the CMS experiment at the LHC,''
  Phys.\ Lett.\ B {\bf 716} (2012) 30
  doi:10.1016/j.physletb.2012.08.021
  [arXiv:1207.7235 [hep-ex]].

\bibitem{atlascms} 
  The ATLAS and CMS Collaborations,
  %``Measurements of the Higgs boson production and decay rates and constraints on its couplings from a combined ATLAS and CMS analysis of the LHC pp collision data at $\sqrt{s}$ = 7 and 8 TeV,''
  ATLAS-CONF-2015-044.

\bibitem{Heinemeyer:2011aa}
  S.~Heinemeyer, O.~Stal and G.~Weiglein,
  %``Interpreting the LHC Higgs Search Results in the MSSM,''
  Phys.\ Lett.\ B {\bf 710} (2012) 201
  doi:10.1016/j.physletb.2012.02.084
  [arXiv:1112.3026 [hep-ph]].

\bibitem{Benbrik:2012rm}
  R.~Benbrik, M.~Gomez Bock, S.~Heinemeyer, O.~Stal, G.~Weiglein and L.~Zeune,
  %``Confronting the MSSM and the NMSSM with the Discovery of a Signal in the two Photon Channel at the LHC,''
  Eur.\ Phys.\ J.\ C {\bf 72} (2012) 2171
  doi:10.1140/epjc/s10052-012-2171-2
  [arXiv:1207.1096 [hep-ph]].
\bibitem{Bechtle:2012jw}
  P.~Bechtle, S.~Heinemeyer, O.~Stal, T.~Stefaniak, G.~Weiglein and L.~Zeune,
  %``MSSM Interpretations of the LHC Discovery: Light or Heavy Higgs?,''
  Eur.\ Phys.\ J.\ C {\bf 73} (2013) 4,  2354
  doi:10.1140/epjc/s10052-013-2354-5
  [arXiv:1211.1955 [hep-ph]].

\bibitem{Ellwanger:2009dp}
  U.~Ellwanger, C.~Hugonie and A.~M.~Teixeira,
  %``The Next-to-Minimal Supersymmetric Standard Model,''
  Phys.\ Rept.\  {\bf 496} (2010) 1
  doi:10.1016/j.physrep.2010.07.001
  [arXiv:0910.1785 [hep-ph]].
\bibitem{Maniatis:2009re}
  M.~Maniatis,
  %``The Next-to-Minimal Supersymmetric extension of the Standard Model reviewed,''
  Int.\ J.\ Mod.\ Phys.\ A {\bf 25} (2010) 3505
  doi:10.1142/S0217751X10049827
  [arXiv:0906.0777 [hep-ph]].
\bibitem{Kang:2012sy}
  Z.~Kang, J.~Li and T.~Li,
  %``On Naturalness of the MSSM and NMSSM,''
  JHEP {\bf 1211} (2012) 024
  doi:10.1007/JHEP11(2012)024
  [arXiv:1201.5305 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP11(2012)024;%%
\bibitem{Vasquez:2012hn}
  D.~A.~Vasquez, G.~Belanger, C.~Boehm, J.~Da Silva, P.~Richardson and C.~Wymant,
  %``The 125 GeV Higgs in the NMSSM in light of LHC results and astrophysics constraints,''
  Phys.\ Rev.\ D {\bf 86} (2012) 035023
  doi:10.1103/PhysRevD.86.035023
  [arXiv:1203.3446 [hep-ph]].
\bibitem{Belanger:2012tt}
  G.~Belanger, U.~Ellwanger, J.~F.~Gunion, Y.~Jiang, S.~Kraml and J.~H.~Schwarz,
  %``Higgs Bosons at 98 and 125 GeV at LEP and the LHC,''
  JHEP {\bf 1301} (2013) 069
  doi:10.1007/JHEP01(2013)069
  [arXiv:1210.1976 [hep-ph]].
\bibitem{King:2012tr}
  S.~F.~King, M.~M\"uhlleitner, R.~Nevzorov and K.~Walz,
  %``Natural NMSSM Higgs Bosons,''
  Nucl.\ Phys.\ B {\bf 870} (2013) 323
  doi:10.1016/j.nuclphysb.2013.01.020
  [arXiv:1211.5074 [hep-ph]].
\bibitem{Badziak:2013bda}
  M.~Badziak, M.~Olechowski and S.~Pokorski,
  %``New Regions in the NMSSM with a 125 GeV Higgs,''
  JHEP {\bf 1306} (2013) 043
  [arXiv:1304.5437 [hep-ph]].
  \bibitem{Christensen:2013dra}
  N.~D.~Christensen, T.~Han, Z.~Liu and S.~Su,
  %``Low-Mass Higgs Bosons in the NMSSM and Their LHC Implications,''
  JHEP {\bf 1308} (2013) 019
  doi:10.1007/JHEP08(2013)019
  [arXiv:1303.2113 [hep-ph]].
\bibitem{Barbieri:2013nka}
  R.~Barbieri, D.~Buttazzo, K.~Kannike, F.~Sala and A.~Tesi,
  %``One or more Higgs bosons?,''
  Phys.\ Rev.\ D {\bf 88} (2013) 055011
  doi:10.1103/PhysRevD.88.055011
  [arXiv:1307.4937 [hep-ph]].
\bibitem{Cao:2013gba}
  J.~Cao, F.~Ding, C.~Han, J.~M.~Yang and J.~Zhu,
  %``A light Higgs scalar in the NMSSM confronted with the latest LHC Higgs data,''
  JHEP {\bf 1311} (2013) 018
  doi:10.1007/JHEP11(2013)018
  [arXiv:1309.4939 [hep-ph]].
\bibitem{Ellwanger:2014dfa}
  U.~Ellwanger and C.~Hugonie,
  %``The semi-constrained NMSSM satisfying bounds from the LHC, LUX and Planck,''
  JHEP {\bf 1408} (2014) 046
  doi:10.1007/JHEP08(2014)046
  [arXiv:1405.6647 [hep-ph]].
\bibitem{Huitu:2014lfa}
  K.~Huitu and H.~Waltari,
  %``Higgs sector in NMSSM with right-handed neutrinos and spontaneous R-parity violation,''
  JHEP {\bf 1411} (2014) 053
  doi:10.1007/JHEP11(2014)053
  [arXiv:1405.5330 [hep-ph]].
\bibitem{King:2014xwa}
  S.~F.~King, M.~M\"uhlleitner, R.~Nevzorov and K.~Walz,
  %``Discovery Prospects for NMSSM Higgs Bosons at the High-Energy Large Hadron Collider,''
  Phys.\ Rev.\ D {\bf 90} (2014) 9,  095014
  doi:10.1103/PhysRevD.90.095014
  [arXiv:1408.1120 [hep-ph]].
\bibitem{Jeong:2014xaa}
  K.~S.~Jeong, Y.~Shoji and M.~Yamaguchi,
  %``Higgs Mixing in the NMSSM and Light Higgsinos,''
  JHEP {\bf 1411} (2014) 148
  doi:10.1007/JHEP11(2014)148
  [arXiv:1407.0955 [hep-ph]].
\bibitem{Guchait:2015owa}
  M.~Guchait and J.~Kumar,
  %``Light Higgs Bosons in NMSSM at the LHC,''
  arXiv:1509.02452 [hep-ph].

\bibitem{Bottino:2011xv}
  A.~Bottino, N.~Fornengo and S.~Scopel,
  %``Phenomenology of light neutralinos in view of recent results at the CERN Large Hadron Collider,''
  Phys.\ Rev.\ D {\bf 85} (2012) 095013
  doi:10.1103/PhysRevD.85.095013
  [arXiv:1112.5666 [hep-ph]].
\bibitem{Boehm:2013gst}
  C.~Boehm, P.~S.~B.~Dev, A.~Mazumdar and E.~Pukartas,
  %``Naturalness of Light Neutralino Dark Matter in pMSSM after LHC, XENON100 and Planck Data,''
  JHEP {\bf 1306} (2013) 113
  doi:10.1007/JHEP06(2013)113
  [arXiv:1303.5386 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP06(2013)113;%%
\bibitem{Belanger:2013pna}
  G.~Belanger, G.~Drieu La Rochelle, B.~Dumont, R.~M.~Godbole, S.~Kraml and S.~Kulkarni,
  %``LHC constraints on light neutralino dark matter in the MSSM,''
  Phys.\ Lett.\ B {\bf 726} (2013) 773
  doi:10.1016/j.physletb.2013.09.059
  [arXiv:1308.3735 [hep-ph]].
\bibitem{Arbey:2013aba}
  A.~Arbey, M.~Battaglia and F.~Mahmoudi,
  %``Supersymmetry with Light Dark Matter confronting the recent CDMS and LHC Results,''
  Phys.\ Rev.\ D {\bf 88} (2013) 095001
  doi:10.1103/PhysRevD.88.095001
  [arXiv:1308.2153 [hep-ph]].
\bibitem{Cao:2013mqa}
  J.~Cao, C.~Han, L.~Wu, P.~Wu and J.~M.~Yang,
  %``A light SUSY dark matter after CDMS-II, LUX and LHC Higgs data,''
  JHEP {\bf 1405} (2014) 056
  doi:10.1007/JHEP05(2014)056
  [arXiv:1311.0678 [hep-ph]].
\bibitem{Beskidt:2014oea}
  C.~Beskidt, W.~de Boer and D.~I.~Kazakov,
  %``The impact of a 126 GeV Higgs on the neutralino mass,''
  Phys.\ Lett.\ B {\bf 738} (2014) 505
  doi:10.1016/j.physletb.2014.08.011
  [arXiv:1402.4650 [hep-ph]].
\bibitem{Han:2014nba}
  T.~Han, Z.~Liu and S.~Su,
  %``Light Neutralino Dark Matter: Direct/Indirect Detection and Collider Searches,''
  JHEP {\bf 1408} (2014) 093
  doi:10.1007/JHEP08(2014)093
  [arXiv:1406.1181 [hep-ph]].  

\bibitem{Kribs:2007ac} 
  G.~D.~Kribs, E.~Poppitz and N.~Weiner,
  %``Flavor in supersymmetry with an extended R-symmetry,''
  Phys.\ Rev.\ D {\bf 78} (2008) 055010
  [arXiv:0712.2039 [hep-ph]].

%\cite{Salam:1974xa}
\bibitem{Salam:1974xa}
  A.~Salam and J.~A.~Strathdee,
  %``Supersymmetry and Fermion Number Conservation,''
  Nucl.\ Phys.\ B {\bf 87} (1975) 85.
  %%CITATION = NUPHA,B87,85;%%
  %158 citations counted in INSPIRE as of 12 Nov 2014
%\cite{Fayet:1974pd}
\bibitem{Fayet:1974pd}
  P.~Fayet,
  %``Supergauge Invariant Extension of the Higgs Mechanism and a Model for the electron and Its Neutrino,''
  Nucl.\ Phys.\ B {\bf 90} (1975) 104.
  %%CITATION = NUPHA,B90,104;%%
  %704 citations counted in INSPIRE as of 12 Nov 2014
  
\bibitem{Dudas:2013gga} 
  E.~Dudas, M.~Goodsell, L.~Heurtier and P.~Tziveloglou,
  %``Flavour models with Dirac and fake gluinos,''
  Nucl.\ Phys.\ B {\bf 884} (2014) 632
  [arXiv:1312.2011 [hep-ph]].
  
%\cite{Kribs:2012gx}
\bibitem{Kribs:2012gx}
  G.~D.~Kribs and A.~Martin,
  %``Supersoft Supersymmetry is Super-Safe,''
  Phys.\ Rev.\ D {\bf 85} (2012) 115014
  [arXiv:1203.4821 [hep-ph]].
  %%CITATION = ARXIV:1203.4821;%%
  %30 citations counted in INSPIRE as of 24 Jul 2013
 %\cite{Chun:2009zx}

\bibitem{Belanger:2009wf}
  G.~Belanger, K.~Benakli, M.~Goodsell, C.~Moura and A.~Pukhov,
  %``Dark Matter with Dirac and Majorana Gaugino Masses,''
  JCAP {\bf 0908} (2009) 027
  [arXiv:0905.1043 [hep-ph]].
  %%CITATION = ARXIV:0905.1043;%%
  %47 citations counted in INSPIRE as of 04 Feb 2015

\bibitem{Chun:2009zx}
  E.~J.~Chun, J.~-C.~Park and S.~Scopel,
  %``Dirac gaugino as leptophilic dark matter,''
  JCAP {\bf 1002} (2010) 015
  [arXiv:0911.5273 [hep-ph]].
  %%CITATION = ARXIV:0911.5273;%%
  %24 citations counted in INSPIRE as of 24 Jul 2013


\bibitem{Buckley:2013sca}
  M.~R.~Buckley, D.~Hooper and J.~Kumar,
  %``Phenomenology of Dirac Neutralino Dark Matter,''
  Phys.\ Rev.\ D {\bf 88} (2013) 063532
  [arXiv:1307.3561].
  %%CITATION = ARXIV:1307.3561;%%
  %23 citations counted in INSPIRE as of 12 Jan 2015
 
\bibitem{Fox:2002bu}
  P.~J.~Fox, A.~E.~Nelson and N.~Weiner,
  %``Dirac gaugino masses and supersoft supersymmetry breaking,''
  JHEP {\bf 0208} (2002) 035
  [hep-ph/0206096].
  %%CITATION = HEP-PH/0206096;%%
 

%\cite{Plehn:2008ae}
\bibitem{Plehn:2008ae}
  T.~Plehn and T.~M.~P.~Tait,
  %``Seeking Sgluons,''
  J.\ Phys.\ G {\bf 36} (2009) 075001
  [arXiv:0810.3919 [hep-ph]].
  %%CITATION = ARXIV:0810.3919;%%
  %113 citations counted in INSPIRE as of 20 Oct 2015
%\cite{Choi:2008ub}
\bibitem{Choi:2008ub}
  S.~Y.~Choi, M.~Drees, J.~Kalinowski, J.~M.~Kim, E.~Popenda and P.~M.~Zerwas,
  %``Color-Octet Scalars of N=2 Supersymmetry at the LHC,''
  Phys.\ Lett.\ B {\bf 672} (2009) 246
  [arXiv:0812.3586 [hep-ph]].
  %%CITATION = ARXIV:0812.3586;%%
  %78 citations counted in INSPIRE as of 20 Oct 2015

%\cite{Choi:2010gc}
\bibitem{Choi:2010gc}
  S.~Y.~Choi, D.~Choudhury, A.~Freitas, J.~Kalinowski, J.~M.~Kim and P.~M.~Zerwas,
  %``Dirac Neutralinos and Electroweak Scalar Bosons of N=1/N=2 Hybrid Supersymmetry at Colliders,''
  JHEP {\bf 1008} (2010) 025
  [arXiv:1005.0818 [hep-ph]].
  %%CITATION = ARXIV:1005.0818;%%
  %24 citations counted in INSPIRE as of 24 Jul 2013

%\cite{Choi:2010an}
\bibitem{Choi:2010an}
  S.~Y.~Choi, D.~Choudhury, A.~Freitas, J.~Kalinowski and P.~M.~Zerwas,
  %``The Extended Higgs System in $R$-symmetric Supersymmetry Theories,''
  Phys.\ Lett.\ B {\bf 697} (2011) 215
   [Erratum-ibid.\ B {\bf 698} (2011) 457]
  [arXiv:1012.2688 [hep-ph]].
  %%CITATION = ARXIV:1012.2688;%%

\bibitem{Benakli:2012cy}
  K.~Benakli, M.~D.~Goodsell and F.~Staub,
  %``Dirac Gauginos and the 125 GeV Higgs,''
  JHEP {\bf 1306} (2013) 073
  [arXiv:1211.0552 [hep-ph]].
  %%CITATION = ARXIV:1211.0552;%%
  %11 citations counted in INSPIRE as of 24 Jul 2013

%\cite{ATLAS:2012ds}
\bibitem{ATLAS:2012ds}
  G.~Aad {\it et al.} [ATLAS Collaboration],
  %``Search for pair-produced massive coloured scalars in four-jet final states with the ATLAS detector in proton-proton collisions at $\sqrt{s}=7$ TeV,''
  Eur.\ Phys.\ J.\ C {\bf 73} (2013) 1,  2263
  [arXiv:1210.4826 [hep-ex]].
  %%CITATION = ARXIV:1210.4826;%%
  %55 citations counted in INSPIRE as of 20 Oct 2015

\bibitem{TheATLAScollaboration:2013jha}
  The ATLAS collaboration [ATLAS Collaboration],
  %``Search for anomalous production of events with same-sign dileptons and $b$ jets in 14.3 fb$^{-1}$ of $pp$ collisions at $\sqrt{s} = 8$ TeV with the ATLAS detector,''
  ATLAS-CONF-2013-051.
  %%CITATION = ATLAS-CONF-2013-051;%%

\bibitem{Kotlarski:2013lja}
  W.~Kotlarski, A.~Kalinowski and J.~Kalinowski,
  %``Searching for Sgluons in the Same-sign Leptons Final State at the LHC,''
  Acta Phys.\ Polon.\ B {\bf 44} (2013) 11,  2149.
  %%CITATION = APPOA,B44,2149;%%

\bibitem{Diessner:2014ksa}
  P.~Diessner, J.~Kalinowski, W.~Kotlarski and D.~St\"ockinger,
  %``Higgs boson mass and electroweak observables in the MRSSM,''
  JHEP {\bf 1412} (2014) 124
  [arXiv:1410.4791 [hep-ph]].
  %%CITATION = ARXIV:1410.4791;%%
  %4 citations counted in INSPIRE as of 12 Jan 2015

\bibitem{Diessner:2015yna}
  P.~Diessner, J.~Kalinowski, W.~Kotlarski and D.~St\"ockinger,
  %``Two-loop correction to the Higgs boson mass in the MRSSM,''
  Adv.\ High Energy Phys.\  {\bf 2015} (2015) 760729
  doi:10.1155/2015/760729
  [arXiv:1504.05386 [hep-ph]].
  %%CITATION = doi:10.1155/2015/760729;%%
  %4 citations counted in INSPIRE as of 24 Nov 2015

\bibitem{Bertuzzo:2014bwa}
  E.~Bertuzzo, C.~Frugiuele, T.~Gregoire and E.~Ponton,
  %``Dirac gauginos, R symmetry and the 125 GeV Higgs,''
  JHEP {\bf 1504} (2015) 089
  [arXiv:1402.5432 [hep-ph]].

% higgs sec    

%\cite{Martin:2015eca}
\bibitem{Martin:2015eca}
  S.~P.~Martin,
  %``Nonstandard supersymmetry breaking and Dirac gaugino masses without supersoftness,''
  Phys.\ Rev.\ D {\bf 92} (2015) 3,  035004
  doi:10.1103/PhysRevD.92.035004
  [arXiv:1506.02105 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.92.035004;%%
  %5 citations counted in INSPIRE as of 17 Nov 2015



\bibitem{Mathematica}
 Wolfram Research, Inc.,
 Mathematica Version 9.0/10.0,
  Champaign, IL (2012/2014) .

\bibitem{SA1}
  F.~Staub,
  %``Sarah,''
  arXiv:0806.0538 [hep-ph].
  %%CITATION = ARXIV:0806.0538;%%
  %82 citations counted in INSPIRE as of 02 Jun 2014

\bibitem{SA2}
  F.~Staub,
  %``From Superpotential to Model Files for FeynArts and CalcHep/CompHep,''
  Comput.\ Phys.\ Commun.\  {\bf 181} (2010) 1077
  [arXiv:0909.2863 [hep-ph]].
  %%CITATION = ARXIV:0909.2863;%%
  %79 citations counted in INSPIRE as of 02 Jun 2014

%\cite{Staub:2010jh}
\bibitem{SA3}
  F.~Staub,
  %``Automatic Calculation of supersymmetric Renormalization Group Equations and Self Energies,''
  Comput.\ Phys.\ Commun.\  {\bf 182} (2011) 808
  [arXiv:1002.0840 [hep-ph]].
  %%CITATION = ARXIV:1002.0840;%%
  %77 citations counted in INSPIRE as of 02 Jun 2014

%\cite{Staub:2012pb}
\bibitem{SA4}
  F.~Staub,
  %``SARAH 3.2: Dirac Gauginos, UFO output, and more,''
    Comput.\ Phys.\ Commun.\  {\bf 184} (2013) 1792 
  [arXiv:1207.0906 [hep-ph]].
  %%CITATION = ARXIV:1207.0906;%%
  %37 citations counted in INSPIRE as of 02 Jun 2014

%\cite{Staub:2013tta}
\bibitem{SA5}
  F.~Staub,
  %``SARAH   4: A tool for (not only SUSY) model builders,''
  Comput.\ Phys.\ Commun.\  {\bf 185} (2014) 1773
  [arXiv:1309.7223 [hep-ph]].
  %%CITATION = ARXIV:1309.7223;%%
  %19 citations counted in INSPIRE as of 02 Jun 2014

%\cite{Goodsell:2014bna}
\bibitem{Goodsell:2014bna}
  M.~D.~Goodsell, K.~Nickel and F.~Staub,
  %``Two-Loop Higgs mass calculations in supersymmetric models beyond the MSSM with SARAH and SPheno,''
  Eur.\ Phys.\ J.\ C {\bf 75} (2015) 1,  32
  [arXiv:1411.0675 [hep-ph]].
  %%CITATION = ARXIV:1411.0675;%%
  %20 citations counted in INSPIRE as of 20 Oct 2015
%\cite{Porod:2003um}
\bibitem{SP1}
  W.~Porod,
  %``SPheno, a program for calculating supersymmetric spectra, SUSY particle decays and SUSY particle production at e+ e- colliders,''
  Comput.\ Phys.\ Commun.\  {\bf 153} (2003) 275
  [hep-ph/0301101].
  %%CITATION = HEP-PH/0301101;%%
  %452 citations counted in INSPIRE as of 02 Jun 2014

%\cite{Porod:2011nf}
\bibitem{SP2}
  W.~Porod and F.~Staub,
  %``SPheno 3.1: Extensions including flavour, CP-phases and models beyond the MSSM,''
  Comput.\ Phys.\ Commun.\  {\bf 183} (2012) 2458
  [arXiv:1104.1573 [hep-ph]].
  %%CITATION = ARXIV:1104.1573;%%
  %108 citations counted in INSPIRE as of 02 Jun 2014

\bibitem{FlexibleSUSY}
  P.~Athron, J.~-h.~Park, D.~St\"ockinger and A.~Voigt,
  %``FlexibleSUSY -- A spectrum generator generator for supersymmetric models,''
  arXiv:1406.2319 [hep-ph].
  %%CITATION = ARXIV:1406.2319;%%
  %1 citations counted in INSPIRE as of 05 Aug 2014


\bibitem{Allanach:2001kg}
  B.~C.~Allanach,
  %``SOFTSUSY: a program for calculating supersymmetric spectra,''
  Comput.\ Phys.\ Commun.\  {\bf 143} (2002) 305
  [hep-ph/0104145].
  %%CITATION = HEP-PH/0104145;%%
  %804 citations counted in INSPIRE as of 19 Aug 2014
  
\bibitem{Allanach:2013kza}
  B.~C.~Allanach, P.~Athron, L.~C.~Tunstall, A.~Voigt and A.~G.~Williams,
  %``Next-to-Minimal SOFTSUSY,''
  Comput.\ Phys.\ Commun.\  {\bf 185} (2014) 2322
  [arXiv:1311.7659 [hep-ph]].
  %%CITATION = ARXIV:1311.7659;%%
  %4 citations counted in INSPIRE as of 16 Oct 2014
  
%\cite{Hahn:2000kx}
\bibitem{FA}
  T.~Hahn,
  %``Generating Feynman diagrams and amplitudes with FeynArts 3,''
  Comput.\ Phys.\ Commun.\  {\bf 140} (2001) 418
  [hep-ph/0012260].
  %%CITATION = HEP-PH/0012260;%%
  %806 citations counted in INSPIRE as of 02 Jun 2014


%\cite{Nejad:2013ina}
\bibitem{FC}
  B.~Chokoufe Nejad, T.~Hahn, J.~-N.~Lang and E.~Mirabella,
  %``FormCalc 8: Better Algebra and Vectorization,''
  arXiv:1310.0274 [hep-ph].
  %%CITATION = ARXIV:1310.0274;%%
  %5 citations counted in INSPIRE as of 02 Jun 2014

\bibitem{Hahn:1998yk}
  T.~Hahn and M.~Perez-Victoria,
  %``Automatized one loop calculations in four-dimensions and D-dimensions,''
  Comput.\ Phys.\ Commun.\  {\bf 118} (1999) 153
  [hep-ph/9807565].
  %%CITATION = HEP-PH/9807565;%%
  %890 citations counted in INSPIRE as of 15 Jul 2014
% HiggsBounds citations
%

\bibitem{HB1}
P.~Bechtle, O.~Brein, S.~Heinemeyer, G.~Weiglein and K.~E.~Williams,
  %``HiggsBounds: Confronting Arbitrary Higgs Sectors with Exclusion Bounds from LEP and the Tevatron,''
  Comput.\ Phys.\ Commun.\  {\bf 181} (2010) 138
  %[arXiv:0811.4169 [hep-ph]].
  %%CITATION = ARXIV:0811.4169;%%
  %174 citations counted in INSPIRE as of 21 Jun 2014

\bibitem{HB2}
P.~Bechtle, O.~Brein, S.~Heinemeyer, G.~Weiglein and K.~E.~Williams,
  %``HiggsBounds 2.0.0: Confronting Neutral and Charged Higgs Sector Predictions with Exclusion Bounds from LEP and the Tevatron,''
  Comput.\ Phys.\ Commun.\  {\bf 182} (2011) 2605
 % [arXiv:1102.1898 [hep-ph]].
  %%CITATION = ARXIV:1102.1898;%%
  %127 citations counted in INSPIRE as of 21 Jun 2014

\bibitem{HB3}
P.~Bechtle, O.~Brein, S.~Heinemeyer, O.~St\aa l, T.~Stefaniak, G.~Weiglein and K.~Williams,
  %``Recent Developments in HiggsBounds and a Preview of HiggsSignals,''
  PoS CHARGED {\bf 2012} (2012) 024
 % [arXiv:1301.2345 [hep-ph]].
  %%CITATION = ARXIV:1301.2345;%%
  %26 citations counted in INSPIRE as of 21 Jun 2014

\bibitem{HB4}
P.~Bechtle, O.~Brein, S.~Heinemeyer, O.~St\aa l, T.~Stefaniak, G.~Weiglein and K.~E.~Williams,
  %``$\mathsf{HiggsBounds}-4$: Improved Tests of Extended Higgs Sectors against Exclusion Bounds from LEP, the Tevatron and the LHC,''
  Eur.\ Phys.\ J.\ C {\bf 74} (2014) 2693
  
%
%  HiggsSignals
%
\bibitem{HS1}
  P.~Bechtle, S.~Heinemeyer, O.~St\aa l, T.~Stefaniak and G.~Weiglein,
  %``$HiggsSignals$: Confronting arbitrary Higgs sectors with measurements at the Tevatron and the LHC,''
  Eur.\ Phys.\ J.\ C {\bf 74} (2014) 2711
  [arXiv:1305.1933 [hep-ph]].
  %%CITATION = ARXIV:1305.1933;%%
  %41 citations counted in INSPIRE as of 30 Jun 2014
  
  \bibitem{HS2}
  O.~St\aa l and T.~Stefaniak,
  %``Constraining extended Higgs sectors with HiggsSignals,''
  PoS EPS {\bf -HEP2013} (2013) 314
  [arXiv:1310.4039 [hep-ph]].
  %%CITATION = ARXIV:1310.4039;%%
  %4 citations counted in INSPIRE as of 30 Jun 2014
  
  
\bibitem{Robens:2015gla}
  T.~Robens and T.~Stefaniak,
  %``Status of the Higgs Singlet Extension of the Standard Model after LHC Run 1,''
  Eur.\ Phys.\ J.\ C {\bf 75} (2015) 104
  doi:10.1140/epjc/s10052-015-3323-y
  [arXiv:1501.02234 [hep-ph]].

\bibitem{Domingo:2015eea}
  F.~Domingo and G.~Weiglein,
  %``NMSSM interpretations of the observed Higgs signal,''
  arXiv:1509.07283 [hep-ph].

%LHC
  

  %\cite{Aad:2014vma}
\bibitem{Aad:2014vma}
  G.~Aad {\it et al.}  [ATLAS Collaboration],
  %``Search for direct production of charginos, neutralinos and sleptons in final states with two leptons and missing transverse momentum in $pp$ collisions at $\sqrt{s} =$ 8 TeV with the ATLAS detector,''
  JHEP {\bf 1405} (2014) 071
  [arXiv:1403.5294 [hep-ex]].
  %%CITATION = ARXIV:1403.5294;%%
  %105 citations counted in INSPIRE as of 24 Apr 2015

\bibitem{Khachatryan:2014mma}
  V.~Khachatryan {\it et al.} [CMS Collaboration],
  %``Searches for electroweak neutralino and chargino production in channels with Higgs, Z, and W bosons in pp collisions at 8 TeV,''
  Phys.\ Rev.\ D {\bf 90} (2014) 9,  092007
  [arXiv:1409.3168 [hep-ex]].
  %%CITATION = ARXIV:1409.3168;%%


\bibitem{Aad:2014yka}
  G.~Aad {\it et al.} [ATLAS Collaboration],
  %``Search for the direct production of charginos, neutralinos and staus in final states with at least two hadronically decaying taus and missing transverse momentum in $pp$ collisions at $\sqrt{s}$ = 8 TeV with the ATLAS detector,''
  JHEP {\bf 1410} (2014) 96
  [arXiv:1407.0350 [hep-ex]].
  %%CITATION = ARXIV:1407.0350;%%
  %40 citations counted in INSPIRE as of 02 Nov 2015


\bibitem{Degrande:2011ua}
  C.~Degrande, C.~Duhr, B.~Fuks, D.~Grellscheid, O.~Mattelaer and T.~Reiter,
  %``UFO - The Universal FeynRules Output,''
  Comput.\ Phys.\ Commun.\  {\bf 183} (2012) 1201
  [arXiv:1108.2040 [hep-ph]].
  %%CITATION = ARXIV:1108.2040;%%
  %238 citations counted in INSPIRE as of 28 Oct 2015

\bibitem{Bahr:2008pv}
  M.~Bahr {\it et al.},
  %``Herwig++ Physics and Manual,''
  Eur.\ Phys.\ J.\ C {\bf 58} (2008) 639
  [arXiv:0803.0883 [hep-ph]].
  %%CITATION = ARXIV:0803.0883;%%
  %1061 citations counted in INSPIRE as of 28 Oct 2015

\bibitem{Bellm:2013hwb}
  J.~Bellm {\it et al.},
  %``Herwig++ 2.7 Release Note,''
  arXiv:1310.6877 [hep-ph].
  %%CITATION = ARXIV:1310.6877;%%
  %54 citations counted in INSPIRE as of 28 Oct 2015
%\cite{Seymour:2013qka}
\bibitem{Seymour:2013qka}
  M.~H.~Seymour and A.~Siodmok,
  %``Constraining MPI models using $\sigma_{eff}$ and recent Tevatron and LHC Underlying Event data,''
  JHEP {\bf 1310} (2013) 113
  [arXiv:1307.5015 [hep-ph]].
  %%CITATION = ARXIV:1307.5015;%%
  %31 citations counted in INSPIRE as of 28 Oct 2015

%\cite{Sherstnev:2007nd}
\bibitem{Sherstnev:2007nd}
  A.~Sherstnev and R.~S.~Thorne,
  %``Parton Distributions for LO Generators,''
  Eur.\ Phys.\ J.\ C {\bf 55} (2008) 553
  [arXiv:0711.2473 [hep-ph]].
  %%CITATION = ARXIV:0711.2473;%%
  %548 citations counted in INSPIRE as of 28 Oct 2015

\bibitem{Drees:2013wra}
  M.~Drees, H.~Dreiner, D.~Schmeier, J.~Tattersall and J.~S.~Kim,
  %``CheckMATE: Confronting your Favourite New Physics Model with LHC Data,''
  Comput.\ Phys.\ Commun.\  {\bf 187} (2014) 227
  [arXiv:1312.2591 [hep-ph]].
  %%CITATION = ARXIV:1312.2591;%%
  %67 citations counted in 

\bibitem{deFavereau:2013fsa}
  J.~de Favereau {\it et al.} [DELPHES 3 Collaboration],
  %``DELPHES 3, A modular framework for fast simulation of a generic collider experiment,''
  JHEP {\bf 1402} (2014) 057
  [arXiv:1307.6346 [hep-ex]].
  %%CITATION = ARXIV:1307.6346;%%
  %322 citations counted in INSPIRE as of 28 Oct 2015

%\cite{Cacciari:2011ma}
\bibitem{Cacciari:2011ma}
  M.~Cacciari, G.~P.~Salam and G.~Soyez,
  %``FastJet User Manual,''
  Eur.\ Phys.\ J.\ C {\bf 72} (2012) 1896
  [arXiv:1111.6097 [hep-ph]].
  %%CITATION = ARXIV:1111.6097;%%
  %1044 citations counted in INSPIRE as of 28 Oct 2015
%\cite{Cacciari:2005hq}
\bibitem{Cacciari:2005hq}
  M.~Cacciari and G.~P.~Salam,
  %``Dispelling the $N^{3}$ myth for the $k_t$ jet-finder,''
  Phys.\ Lett.\ B {\bf 641} (2006) 57
  [hep-ph/0512210].
  %%CITATION = HEP-PH/0512210;%%
  %1233 citations counted in INSPIRE as of 28 Oct 2015
%\cite{Cacciari:2008gp}
\bibitem{Cacciari:2008gp}
  M.~Cacciari, G.~P.~Salam and G.~Soyez,
  %``The Anti-k(t) jet clustering algorithm,''
  JHEP {\bf 0804} (2008) 063
  [arXiv:0802.1189 [hep-ph]].
  %%CITATION = ARXIV:0802.1189;%%
  %3114 citations counted in INSPIRE as of 28 Oct 2015
%\cite{Read:2002hq}
\bibitem{Read:2002hq}
  A.~L.~Read,
  %``Presentation of search results: The CL(s) technique,''
  J.\ Phys.\ G {\bf 28} (2002) 2693.
  %%CITATION = JPAGA,G28,2693;%%
  %1224 citations counted in INSPIRE as of 28 Oct 2015

  
%\cite{TheATLAScollaboration:2013hha}
\bibitem{TheATLAScollaboration:2013hha}
  The ATLAS collaboration [ATLAS Collaboration],
  %``Search for direct-slepton and direct-chargino production in final states with two opposite-sign leptons, missing transverse momentum and no jets in 20/fb of pp collisions at sqrt(s) = 8 TeV with the ATLAS detector,''
  ATLAS-CONF-2013-049.
  %%CITATION = ATLAS-CONF-2013-049;%%
  %90 citations counted in INSPIRE as of 28 Oct 2015

\bibitem{ATLAS:2013rla}
  [ATLAS Collaboration],
  %``Search for direct production of charginos and neutralinos in events with three leptons and missing transverse momentum in 21$\,$fb$^{-1}$ of pp collisions at $\sqrt{s}=8\,$TeV with the ATLAS detector,''
  ATLAS-CONF-2013-035.
  %%CITATION = ATLAS-CONF-2013-035;%%
  %101 citations counted in INSPIRE as of 28 Oct 2015

  %\cite{Aad:2014nua}
\bibitem{Aad:2014nua}
  G.~Aad {\it et al.}  [ATLAS Collaboration],
  %``Search for direct production of charginos and neutralinos in events with three leptons and missing transverse momentum in $\sqrt{s} =$ 8TeV $pp$ collisions with the ATLAS detector,''
  JHEP {\bf 1404} (2014) 169
  [arXiv:1402.7029 [hep-ex]].
  %%CITATION = ARXIV:1402.7029;%%
  %85 citations counted in INSPIRE as of 24 Apr 2015
  
\bibitem{ATLAS:2013qla}
  [ATLAS Collaboration],
  %``Search for supersymmetry in events with four or more leptons in 21$\,$fb$^{-1}$ of pp collisions at $\sqrt{s}=8\,$TeV with the ATLAS detector,''
  ATLAS-CONF-2013-036.
  %%CITATION = ATLAS-CONF-2013-036;%%
  %46 citations counted in INSPIRE as of 28 Oct 2015

\bibitem{Alwall:2014hca}
  J.~Alwall {\it et al.},
  %``The automated computation of tree-level and next-to-leading order differential cross sections, and their matching to parton shower simulations,''
  JHEP {\bf 1407} (2014) 079
  [arXiv:1405.0301 [hep-ph]].
  %%CITATION = ARXIV:1405.0301;%%
  %540 citations counted in INSPIRE as of 28 Oct 2015

%\cite{Belyaev:2012qa}
\bibitem{Belyaev:2012qa}
  A.~Belyaev, N.~D.~Christensen and A.~Pukhov,
  %``CalcHEP 3.4 for collider physics within and beyond the Standard Model,''
  Comput.\ Phys.\ Commun.\  {\bf 184} (2013) 1729
  [arXiv:1207.6082 [hep-ph]].
  %%CITATION = ARXIV:1207.6082;%%
  %260 citations counted in INSPIRE as of 19 Oct 2015


\bibitem{Aad:2015jqa}
  G.~Aad {\it et al.} [ATLAS Collaboration],
  %``Search for direct pair production of a chargino and a neutralino decaying to the 125 GeV Higgs boson in $\sqrt{s} = 8$  TeV ${pp}$ collisions with the ATLAS detector,''
  Eur.\ Phys.\ J.\ C {\bf 75} (2015) 5,  208
  [arXiv:1501.07110 [hep-ex]].
  %%CITATION = ARXIV:1501.07110;%%



  %\cite{Belanger:2014vza}
\bibitem{Belanger:2014vza}
  G.~Belanger, F.~Boudjema, A.~Pukhov and A.~Semenov,
  %``micrOMEGAs4.1: two dark matter candidates,''
  Comput.\ Phys.\ Commun.\  {\bf 192} (2015) 322
  [arXiv:1407.6129 [hep-ph]].
  %%CITATION = ARXIV:1407.6129;%%
  %35 citations counted in INSPIRE as of 19 Oct 2015

\bibitem{Savage:2015xta}
  C.~Savage, A.~Scaffidi, M.~White and A.~G.~Williams,
  %``LUX likelihood and limits on spin-independent and spin-dependent WIMP couplings with LUXCalc,''
  arXiv:1502.02667 [hep-ph].
  %%CITATION = ARXIV:1502.02667;%%
  
\bibitem{Akerib:2012ys}
  D.~S.~Akerib {\it et al.}  [LUX Collaboration],
  %``The Large Underground Xenon (LUX) Experiment,''
  Nucl.\ Instrum.\ Meth.\ A {\bf 704} (2013) 111
  [arXiv:1211.3788 [physics.ins-det]].
  %%CITATION = ARXIV:1211.3788;%%
  %87 citations counted in INSPIRE as of 12 Feb 2015

  %\cite{Agashe:2014kda}
\bibitem{Agashe:2014kda}
  K.~A.~Olive {\it et al.} [Particle Data Group Collaboration],
  %``Review of Particle Physics,''
  Chin.\ Phys.\ C {\bf 38} (2014) 090001.
  %%CITATION = CHPHD,C38,090001;%%
  %2115 citations counted in INSPIRE as of 19 Oct 2015

  \bibitem{Ade:2013zuv}
  P.~A.~R.~Ade {\it et al.}  [Planck Collaboration],
  %``Planck 2013 results. XVI. Cosmological parameters,''
  Astron.\ Astrophys.\  {\bf 571} (2014) A16
  [arXiv:1303.5076 [astro-ph.CO]].
  %%CITATION = ARXIV:1303.5076;%%
  %3076 citations counted in INSPIRE as of 13 Feb 2015

